Data-driven confidence bands for distributed nonparametric regression

Gaussian Process Regression and Kernel Ridge Regression are popular nonparametric regression approaches. Unfortunately, they suffer from high computational complexity rendering them inapplicable to the modern massive datasets. To that end a number of approximations have been suggested, some of them allowing for a distributed implementation. One of them is the divide and conquer approach, splitting the data into a number of partitions, obtaining the local estimates and finally averaging them. In this paper we suggest a novel computationally efficient fully data-driven algorithm, quantifying uncertainty of this method, yielding frequentist $L_2$-confidence bands. We rigorously demonstrate validity of the algorithm. Another contribution of the paper is a minimax-optimal high-probability bound for the averaged estimator, complementing and generalizing the known risk bounds.

==> code/venv/bin/activate <==
# This file must be used with "source bin/activate" *from bash*
# you cannot run it directly

deactivate () {
    # reset old environment variables
    if [ -n "${_OLD_VIRTUAL_PATH:-}" ] ; then
        PATH="${_OLD_VIRTUAL_PATH:-}"
        export PATH
        unset _OLD_VIRTUAL_PATH
    fi
    if [ -n "${_OLD_VIRTUAL_PYTHONHOME:-}" ] ; then
        PYTHONHOME="${_OLD_VIRTUAL_PYTHONHOME:-}"
        export PYTHONHOME
        unset _OLD_VIRTUAL_PYTHONHOME
    fi

    # This should detect bash and zsh, which have a hash command that must
    # be called to get it to forget past commands.  Without forgetting
    # past commands the $PATH changes we made may not be respected
    if [ -n "${BASH:-}" -o -n "${ZSH_VERSION:-}" ] ; then
        hash -r
    fi

    if [ -n "${_OLD_VIRTUAL_PS1:-}" ] ; then
        PS1="${_OLD_VIRTUAL_PS1:-}"
        export PS1
        unset _OLD_VIRTUAL_PS1
    fi

    unset VIRTUAL_ENV
    if [ ! "${1:-}" = "nondestructive" ] ; then
    # Self destruct!
        unset -f deactivate
    fi
}

# unset irrelevant variables
deactivate nondestructive

VIRTUAL_ENV="/Users/avanesov/sfb/gprConsistency/code/venv"
export VIRTUAL_ENV

_OLD_VIRTUAL_PATH="$PATH"
PATH="$VIRTUAL_ENV/bin:$PATH"
export PATH

# unset PYTHONHOME if set
# this will fail if PYTHONHOME is set to the empty string (which is bad anyway)
# could use `if (set -u; : $PYTHONHOME) ;` in bash
if [ -n "${PYTHONHOME:-}" ] ; then
    _OLD_VIRTUAL_PYTHONHOME="${PYTHONHOME:-}"
    unset PYTHONHOME
fi

if [ -z "${VIRTUAL_ENV_DISABLE_PROMPT:-}" ] ; then
    _OLD_VIRTUAL_PS1="${PS1:-}"
    if [ "x(venv) " != x ] ; then
	PS1="(venv) ${PS1:-}"
    else
    if [ "`basename \"$VIRTUAL_ENV\"`" = "__" ] ; then
        # special case for Aspen magic directories
        # see http://www.zetadev.com/software/aspen/
        PS1="[`basename \`dirname \"$VIRTUAL_ENV\"\``] $PS1"
    else
        PS1="(`basename \"$VIRTUAL_ENV\"`)$PS1"
    fi
    fi
    export PS1
fi

# This should detect bash and zsh, which have a hash command that must
# be called to get it to forget past commands.  Without forgetting
# past commands the $PATH changes we made may not be respected
if [ -n "${BASH:-}" -o -n "${ZSH_VERSION:-}" ] ; then
    hash -r
fi


==> code/venv/bin/easy_install <==
#!/Users/avanesov/sfb/gprConsistency/code/venv/bin/python
# EASY-INSTALL-ENTRY-SCRIPT: 'setuptools==40.8.0','console_scripts','easy_install'
__requires__ = 'setuptools==40.8.0'
import re
import sys
from pkg_resources import load_entry_point

if __name__ == '__main__':
    sys.argv[0] = re.sub(r'(-script\.pyw?|\.exe)?$', '', sys.argv[0])
    sys.exit(
        load_entry_point('setuptools==40.8.0', 'console_scripts', 'easy_install')()
    )


==> code/venv/bin/easy_install-3.7 <==
#!/Users/avanesov/sfb/gprConsistency/code/venv/bin/python
# EASY-INSTALL-ENTRY-SCRIPT: 'setuptools==40.8.0','console_scripts','easy_install-3.7'
__requires__ = 'setuptools==40.8.0'
import re
import sys
from pkg_resources import load_entry_point

if __name__ == '__main__':
    sys.argv[0] = re.sub(r'(-script\.pyw?|\.exe)?$', '', sys.argv[0])
    sys.exit(
        load_entry_point('setuptools==40.8.0', 'console_scripts', 'easy_install-3.7')()
    )


==> code/venv/bin/pip <==
#!/Users/avanesov/sfb/gprConsistency/code/venv/bin/python
# EASY-INSTALL-ENTRY-SCRIPT: 'pip==19.0.3','console_scripts','pip'
__requires__ = 'pip==19.0.3'
import re
import sys
from pkg_resources import load_entry_point

if __name__ == '__main__':
    sys.argv[0] = re.sub(r'(-script\.pyw?|\.exe)?$', '', sys.argv[0])
    sys.exit(
        load_entry_point('pip==19.0.3', 'console_scripts', 'pip')()
    )


==> code/venv/bin/pip3 <==
#!/Users/avanesov/sfb/gprConsistency/code/venv/bin/python
# EASY-INSTALL-ENTRY-SCRIPT: 'pip==19.0.3','console_scripts','pip3'
__requires__ = 'pip==19.0.3'
import re
import sys
from pkg_resources import load_entry_point

if __name__ == '__main__':
    sys.argv[0] = re.sub(r'(-script\.pyw?|\.exe)?$', '', sys.argv[0])
    sys.exit(
        load_entry_point('pip==19.0.3', 'console_scripts', 'pip3')()
    )


==> code/venv/bin/pip3.7 <==
#!/Users/avanesov/sfb/gprConsistency/code/venv/bin/python
# EASY-INSTALL-ENTRY-SCRIPT: 'pip==19.0.3','console_scripts','pip3.7'
__requires__ = 'pip==19.0.3'
import re
import sys
from pkg_resources import load_entry_point

if __name__ == '__main__':
    sys.argv[0] = re.sub(r'(-script\.pyw?|\.exe)?$', '', sys.argv[0])
    sys.exit(
        load_entry_point('pip==19.0.3', 'console_scripts', 'pip3.7')()
    )


==> dncproof.tex <==
%!TEX root = main.tex
\section{Proof of $\bar f$ consistency}\label{fbarsec}
Denote a map from $\X$ to $\R^{\infty}$
\begin{equation}
  \psi(X) \coloneqq \brac{\sqrt{\mu_1}\phi_1(X)~~ \sqrt{\mu_2}\phi_2(X)~~ \sqrt{\mu_3}\phi_3(X)~~ ... }^T \in \R^{\infty}
\end{equation}
and  $\psi_i \coloneqq  \psi(X_i)$.

We have earlier introduced objects related to the global estimator $\fhat$, such as $\Psi$, $\DrhoSq$, $\hatparam$, $\fhatbold$. In this section we make use of their local counterparts related to $\fhatm$ like $\Psim$, $\DrhomSq$, $\hatparamm$, $\fhatboldm$,  Also define $\barparam \coloneqq \frac{1}{P} \sum_p \hatparamm$ and $\fbarbold \coloneqq \frac{1}{P}\sum_p \fhatboldm$. Throughout the section we let $\snull \ge s$. 
\begin{lemma}\label{fhatgar}
   Consider a centered Gaussian element of a Hilbert space $\ghat$ with a covariance operator
   \begin{equation}
     \Var{\ghat} = \sigma^2\brac{M^2+\rho I}^{-1} M^2.
   \end{equation}
  Then for all positive $\t > 2.6$ uniformly for $r>0$
   \begin{equation}
     \abs{\Prob{\norm{\Drho\brac{\hatparam - \trueparamrho}} \le r} - \Prob{n^{-1/2}\norm{\ghat}\le r}} \le \C \brac{\delta(n, \t) + \frac{\g^3}{\sigma^3} n^{-1/2}} + 4e^{-\t/2},
   \end{equation}
   where $\delta$ comes from \ref{lemmadesign}.
   
\end{lemma}
\begin{proof}
  Using Fisher expansion (which holds in the form of equality for quadratic likelihoods and Gaussian priors)
  \begin{equation}
    \Drho\brac{\hatparam - \trueparamrho} = \frac{1}{n} \DrhoInv \Psit \eps
  \end{equation}
  or alternatively
  \begin{equation}
    \Drho\brac{\hatparam - \trueparamrho} = \frac{1}{n} \DrhoInv \brac{\sum_{i=1}^n \psi_i \varepsilon_i}.
  \end{equation}
  Denote the set which the implication of \ref{lemmadesign} holds on as $\Omega$ driven by $\t > 2.6$: $\Omega = \Omega(\t)$ of measure at least $1-e^{-\t/2}$. On this set 
  \begin{equation}
     (1+\delta)^{-1} (M^2+\rho I)^{-1} \le \DrhoSqInv \le (1-\delta)^{-1} (M^2+\rho I)^{-1}
  \end{equation}
  and hence for a positive $r$
  \begin{equation}\label{conduncondfhat}
  \begin{split}
    &\Prob{\norm{\frac{1}{n} \DrhoInv \brac{\sum_{i=1}^n \psi_i \varepsilon_i}} \le r} \le \Prob{\norm{\frac{1}{n} \DrhoInv \brac{\sum_{i=1}^n \psi_i \varepsilon_i}} \le r \given \Omega(\t)} + 2e^{-\t/2}  \\
    & \le \Prob{\norm{\frac{1}{n \sqrt{1+\delta}} \brac{M^2+\rho I}^{-1/2} \brac{\sum_{i=1}^n \psi_i \varepsilon_i} } \le r \given \Omega(\t)} + 2  e^{-\t/2} \\
    &\le \Prob{\norm{\frac{1}{n\sqrt{1+\delta}} \brac{M^2+\rho I}^{-1/2} \brac{\sum_{i=1}^n \psi_i \varepsilon_i} } \le r} + 4 e^{-\t/2},
  \end{split}
  \end{equation}
  where we have also used \ref{condlemma} twice. Note, $\psi_i \varepsilon_i$ are i.i.d. and $\Var{\psi_i\varepsilon_i} = M^2$ as $\psi_i$ are orthonormal eigenfunctions. Further, using \ref{effdimlemma}
    \begin{equation}
    \E{\norm{\brac{M^2+\rho I }^{-1/2} \psi_i \varepsilon_i}^2} \asymp \sigma^2 \sum_j \frac{\mu_j}{\mu_j+\rho} \asymp \C \sigma^2 \rho^{-1/(2s)}
  \end{equation}
  and using Jensen inequality, sub-Gaussianity (to bound the $6$-th moment) and \ref{effdimlemma} again
  \begin{equation}
    \E{\norm{\brac{M^2+\rho I }^{-1/2} \psi_i \varepsilon_i}^3} \le \phiinf^3 \sqrt{\E{\varepsilon_i^6}} \brac{\sum_j \frac{\mu_j}{\mu_j+\rho}}^{3/2}\le \C  \g^3 \brac{\rho^{-1/(2s)}}^{3/2}.
  \end{equation}
  
  Now we are ready to employ the Central Limit Theorem \ref{cltlemma}. Consider a Gaussian element in a Hilbert space $\gdelta$. Let it be centered and its covariance operator be
  \begin{equation}
    \Var{\gdelta} = \frac{\sigma^2}{(1+\delta)} \brac{M^2+\rho I}^{-1/2} M^2 \brac{M^2+\rho I}^{-1/2}.
  \end{equation}
  Then for all positive $r$ uniformly
  \begin{equation}\label{GARfhat}
    \Prob{\norm{\frac{1}{\sqrt{n(1+\delta)}} \brac{M^2+\rho I}^{-1/2} \brac{\sum_{i=1}^n \psi_i \varepsilon_i} } \le r} \le \Prob{\norm{\gdelta} < r} +  \frac{\C \g^3}{\sigma^3}n^{-1/2}.
  \end{equation}
  Now we bound the discrepancy between the distributions of $\gdelta$ and $\ghat$ using \ref{gcomp} and the fact that $\delta < 1$
  \begin{equation}\label{gcrfhat}
    \sup_r\abs{\Prob{\norm{\ghat} \le r} - \Prob{\norm{\gdelta} \le r}} \le \C \delta.
  \end{equation}
  Combination of \eqref{conduncondfhat}, \eqref{GARfhat} and \eqref{gcrfhat} yields uniformly for all positive $r$
  \begin{equation}
    \Prob{\norm{\frac{1}{n} \DrhoInv \brac{\sum_{i=1}^n \psi_i \varepsilon_i}} \le r} \le \Prob{n^{-1/2}\norm{\ghat}\le r} + \C \brac{\delta + \frac{\g^3}{\sigma^3} n^{-1/2}} + 4e^{-\t/2}. 
  \end{equation}
  In the same way one can obtain the lower bound
  \begin{equation}
    \Prob{\norm{\frac{1}{n} \DrhoInv \brac{\sum_{i=1}^n \psi_i \varepsilon_i}} \le r} \ge \Prob{n^{-1/2}\norm{\ghat}\le r} - \C \brac{\delta +\frac{\g^3}{\sigma^3} n^{-1/2}} - 4e^{-\t/2}. 
  \end{equation}
\end{proof}

\begin{lemma}\label{fbargar}
  Consider a centered Gaussian element of a Hilbert space $\gbar$ with a covariance operator
  \begin{equation}
    \Var{\gbar} = \sigma^2\brac{M^2+\rho I}^{-1} M^2.
  \end{equation}
 Then for all positive $\t > 2.6$ uniformly for positive $r$
  \begin{equation}
  \begin{split}
    \abs{\Prob{\norm{\brac{M^2+\rho I}^{1/2}\brac{\barparam-\trueparamrho}} \le r} - \Prob{n^{-1/2}\norm{\gbar}\le r}} \\\le \C \brac{\delta(S, \t) + \frac{\g^3}{\sigma^3}n^{-1/2}} + 4Pe^{-\t/2},
  \end{split}
  \end{equation}
  where $\delta$ comes from \ref{lemmadesign}.
\end{lemma}
\begin{proof}
  The strategy of the proof is similar to that of \ref{fhatgar}.
  Again,
  \begin{equation}
    \Drhom\brac{\hatparamm - \trueparamrho} = \frac{1}{S} \DrhomInv \brac{\sum_{i\in S_p} \psi_i \varepsilon_i}.
  \end{equation}
  Apply \ref{lemmadesign} $P$ times and obtain on a set $\Omega(\t)$ of probability at least $1-Pe^{-\t/2}$
  \begin{equation}
     (1+\delta)^{-1} (M^2+\rho I)^{-1} \le \DrhomSqInv \le (1-\delta)^{-1} (M^2+\rho I)^{-1},
  \end{equation}
  where $\delta = \delta(S, \t)$.
  Hence on this set we have
  \begin{equation}
    \brac{M^2+\rho I}^{1/2} \brac{\barparam - \trueparamrho} \ge \frac{1}{n \brac{1+\delta}} \brac{M^2+\rho I}^{-1/2} \sum_{i=1}^n \psi_i \varepsilon_i  .
  \end{equation}
  Consider a centered Gaussian element in a Hilbert space $\gdelta$ with covariance operator 
  \begin{equation}
    \Var{\gdelta} = \frac{1}{(1+\delta)^2} \brac{M^2+\rho I}^{-1/2} M^2 \brac{M^2+\rho I}^{-1/2}.
  \end{equation}
  \ref{cltlemma} yields
  \begin{equation}
    \Prob{\norm{\frac{1}{\sqrt{n}(1+\delta)} \brac{M^2+\rho I}^{-1/2} \brac{\sum_{i=1}^n \psi_i \varepsilon_i} } \le r} \le \Prob{\norm{\gdelta} < r} + \C\frac{\g^3}{\sigma^3} n^{-1/2}.
  \end{equation}
  Gaussian Comparison (\ref{gcomp}) of $\gdelta$ and $\gbar$ completes the proof.
\end{proof}
Now we are ready to combine the two Gaussian approximations thus demonstrating the deviation bound for $\fbar$.
\begin{proof}[Proof of \ref{fbarth}]
  Apply \ref{fhatgar} and \ref{fbargar}. Notice $\gbar$ and $\ghat$ have the same distribution. Hence, uniformly for $r>0$
  \begin{equation}
    \abs{\Prob{\norm{\brac{M^2+\rho I}^{1/2}\brac{\barparam-\trueparamrho}} \le r} - \Prob{\norm{\Drho\brac{\hatparam - \trueparamrho}} \le r}} \le R,
  \end{equation}
  where 
  \begin{equation}
    R \coloneqq  \C \brac{\delta(n, \t)+ \delta(S, \t) + \frac{\g^3}{\sigma^3}n^{-1/2}} + 4(P+1)e^{-\t/2}.
  \end{equation}
  Applying \ref{scoreconcentration} and \ref{spokpanov} (in the same way as in the proof of \ref{maintheorem}) we obtain
  \begin{equation}
    {\norm{\brac{M^2+\rho I}^{1/2}\brac{\barparam-\trueparamrho}} \le  \C\g\sqrt{\frac{\brac{1+\sqrt{\x}+2\x}}{\rho^{1/(2s)}n(1-\delta(n, \t))} }} 
  \end{equation}
  on a set of probability at least $1-e^{-\x} - R$
  and hence, using the fact that $M^2+\rho I \ge M^2$
  \begin{equation}
    \Prob{{\norm{M\brac{\barparam-\trueparamrho}} \le  \C\g\sqrt{\frac{\brac{1+\sqrt{\x}+2\x}}{\rho^{1/(2s)}n(1-\delta(n,\t))} }} }\ge 1-1-e^{-\x} - R.
  \end{equation}
  Finally we obtain a bound for the bias term $\norm{\ftrueboldrho - \ftruebold}$ using \ref{biaslemma}
   and complete the proof choosing $\x=\t=4 \log n$.
\end{proof}


==> errinvaricommands.tex <==
\newcommand{\zstari}{z^*_i}
\newcommand{\fbold}{\boldsymbol{f}}
\newcommand{\zbold}{\boldsymbol{z}}
\newcommand{\zstarbold}{\boldsymbol{z^*}}
\newcommand{\ybold}{\boldsymbol{y}}
\newcommand{\xbold}{\boldsymbol{x}}
\newcommand{\sigmaeps}{\sigma_{\varepsilon}}
\newcommand{\sigmaxi}{\sigma_{\xi}}
\newcommand{\fstarbbold}{\boldsymbol{f^*}}
\newcommand{\hatfbold}{\boldsymbol{\hat f}}
\newcommand{\hatzbold}{\boldsymbol{\hat z}}
\newcommand{\starfboldrho}{\boldsymbol{f^*_\rho}}
\newcommand{\starzboldrho}{\boldsymbol{z^*_\rho}}
\newcommand{\starfrho}{{f^*_\rho}}


